Effects of baryons on the gravitational redshift profile of {\Lambda}CDM halos

Gravitational redshifts and other relativistic effects are beginning to be studied in the context of galaxy clustering. Distortions consistent with those expected in General Relativity have been measured in galaxy cluster redshift profiles by Wojtak et al. and others and in the the cross-correlation function of galaxy populations by Alam et al. On scales below ~20 Mpc/$h$ simulations have shown that gravitational redshift dominates over other effects. However, this signal is related to the shape and depth of gravitational potentials, and therefore the matter density in galaxies and galaxy clusters that is responsible for them. We investigate the effects of baryonic physics on the gravitational redshift profiles of massive (group and cluster-sized) halos. We compare the profiles of different components in halos taken from the MassiveBlack-II cosmological hydrodynamic simulation and a dark matter-only version of the same simulation. We find that inclusion of baryons, cooling, star formation and feedback significantly alters the relevant inner density profiles. These baryonic effects lead to overall increases in both gravitational redshifts and the transverse relativistic Doppler effects by up to ~50% for group size halos. We show how modified Navarro Frenk White halo profiles can be used to parametrize these differences, and provide relevant halo profile fits.

==> tex/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\subsection{Gravitational potentials of subhalos}
The signal of the shell estimator is really sensitive to the gravitational potentials assigned to each subhalo. From simulations we have potentials of the particles in each subhalo, the question is what could be potentials of subhalos. All previous figures take the mean potential of all particles belonging to a subhalo as the potential of the subhalo which clearly suppresses the signal of the gravitational redshift effect. Another choice is to use the potential of the most bound particle inside each subhalo. As can be seen from the contours of the top left panel in Fig.~\ref{fig:sliceplot}, the bound particles around the center would be approximately twice as the average potential inside those subhalos thus double the signal.

However, the discussion above only comes from the large-scale structure information. The signal can be even boosted by the structure information of galaxies. Here we use the analytic profile of the galaxy from \cite{cappi1995} Eqn. 7,
\begin{equation}\label{eq:cappi}
V(r) \simeq \frac {GM} {cR_0}\left[1+\ln\left(\frac {R_0} R\right)\right] \simeq 10^{-5}\sigma^2\left[1+\ln\left(\frac {R_0} R\right)\right]
\end{equation}
where $R_0=3R_e$ and $R_e$ is the half-mass radius. As is pointed out by Cappi, this is a good approximation of the projected gravitational potential profile within the range $0.05R_e<R<3R_e$. The signal of the shell estimator could be enlarged by adding this additional galaxy potential since the velocity dispersion $\sigma$ is positively correlated with the subhalo mass and the gravitational redshift.

\begin{figure}
  \centering
    \includegraphics[width=0.5\textwidth]{./plots/cappi_3000.png}
     \caption{Shell estimators of different subhalo potentials. We only exam the gravitational redshift effects here. The red curve shows the subhalo potential as the mean potential of all the particles inside. The green curve shows the subhalo potential as the potential of the most bound particle inside. The blue and cyan curves add the galaxy structure using Eqn.~\ref{eq:cappi} onto the red and green curves respectively. The error bars are the errors on the mean.}
     \label{fig:galaxy_lss}
\end{figure}

Fig.~\ref{fig:galaxy_lss} shows the how different potential values of subhalos affect the shell estimator. We can see by adding galaxy structure information onto large-scale structure, the signals scale up, which indicates most of the signal comes from the galaxy inner structures instead of the large-scale information.


\subsection{Resolution test}
The resolution of the simulation can affect the shell estimator as well. If the simulation cannot resolve the subhalos very well, the signal will also be suppressed. We construct a resolution test by doubling, tripling and quadrupling the number of particles along each dimension and then compare the $z_\mathrm{g}$s of the same subhalos between different resolutions. We match two subhalos according to their positions. Fig.~\ref{fig:res} illustrates that our resolution basically converges with higher resolutions though higher resolutions would be better.
\begin{figure}
  \centering
    \includegraphics[width=0.5\textwidth]{/Users/Hongyu/Documents/for_rupert/res.png}
     \caption{Resolution test of different subhalo potentials. The left panel shows the resolution test of mean gravitational potentials of all the particles inside subhalos. The right panel shows the resolution test of potentials of the most bound particles inside subhalos. The curves are the redshift ratios of two different resolutions. We use our current resolution as the base case (denominators) and higher resolutions as the comparison (numerators).}
     \label{fig:res}
\end{figure}

\section{Conclusions}
Using the $N$-body simulations, we have generally modeled different effects existing in the observations and made predictions for these relative effects between pairs of galaxies in high mass and low mass subsets as a function of scale in redshift space. We have shown the distortions in galaxy cross-correlation functions and quantified the line-of-sight asymmetries of them. We've also compared our results and found consistency with CMASS data. Finally, we have discussed the aspects which are capable of affecting signals. Our conclusions are the following:
\begin{enumerate}
\item
Relativistic effects are a new probe of galaxies and large-scale structure.
\item
All of the four effects (the gravitational redshift effect, the TD effect, the LC bias and the SRB effect) lead to asymmetries on the cross-correlation functions but these asymmetries are different. By studying the defined shell estimator, the signal is largely affected by the gravitational redshift effect at small scales and the SRB effect at large scales.
\item
Most of the signals actually come from the galaxy structure information instead of the large-scale information. Future projects with MaNGA will unveil the potential profiles inside galaxies.
\end{enumerate}


\section*{Acknowledgments}
This work was supported by NSF Award 1412966. I would like to thank Rupert A.C. Croft for the use of the \textsc{P-Gadget3} code. I would also like to thank ... for useful discussions.

